Automatic Creation of Named Entity Recognition Datasets by Querying Phrase Representations

Most weakly supervised named entity recognition (NER) models rely on domain-specific dictionaries provided by experts. This approach is infeasible in many domains where dictionaries do not exist. While a phrase retrieval model was used to construct pseudo-dictionaries with entities retrieved from Wikipedia automatically in a recent study, these dictionaries often have limited coverage because the retriever is likely to retrieve popular entities rather than rare ones. In this study, we present a novel framework, HighGEN, that generates NER datasets with high-coverage pseudo-dictionaries. Specifically, we create entity-rich dictionaries with a novel search method, called phrase embedding search, which encourages the retriever to search a space densely populated with various entities. In addition, we use a new verification process based on the embedding distance between candidate entity mentions and entity types to reduce the false-positive noise in weak labels generated by high-coverage dictionaries. We demonstrate that HighGEN outperforms the previous best model by an average F1 score of 4.7 across five NER benchmark datasets.

==> tables/ablation.tex <==
\begin{table}[t!]
\centering
\footnotesize
\begin{adjustbox}{max width = 0.99\columnwidth}

\begin{tabular}{lccc}
\toprule
\textbf{Model} & \textbf{CoNLL-2003} & \textbf{BC5CDR} \\
\midrule
\multicolumn{3}{l}{\textit{Unlabeled sentences (with the same pseudo-dictionary)}} \\
\quad Only $\mathbf{X}_2$ ($k_l = |\mathbf{X}_1|$) &  & \\
\quad Only $\mathbf{X}_2$ ($k_l = \text{30k}$) &  & \\
\quad $\mathbf{X}_1$ + $\mathbf{X}_2$ ($k_l = \text{5k}$) &  & \\
\quad $\mathbf{X}_1$ + $\mathbf{X}_2$ ($k_l = \text{30k}$) &  & \\
\quad Only $\mathbf{X}_1$ ({HighGEN}) & \\
\midrule
\ours~w/o Verification \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Ablation study.}
\label{table:ablation}
\end{table}

==> tables/ablation_of_emb.tex <==
\begin{table}[t]
\centering
\footnotesize

\begin{adjustbox}{max width = 0.99\columnwidth}

\begin{tabular}{lccc}
\toprule
\textbf{Model} & \begin{tabular}[c]{@{}c@{}} \textbf{CoNLL} \\ \textbf{-2003} \end{tabular} & \begin{tabular}[c]{@{}c@{}} \textbf{NCBI-} \\ \textbf{disease} \end{tabular} & \textbf{CHEMDNER} \\
\midrule
\ours & \textbf{73.6} & \textbf{71.9} & \textbf{63.4} \\
\quad w/o Embed. & 70.3 & 69.0 & 58.2 \\
\midrule
\gener & 71.5 & 67.2 & 61.8 \\
\bottomrule
\end{tabular}
\end{adjustbox}
%\textbf{77.6}
%76.6
%73.4
\caption{
Ablation study of embedding matching.
We report F1 scores of self-training models on the validation sets.
\textbf{Embed.}: embedding matching.
}
\label{tab:ablation_of_emb}
\end{table}

==> tables/bond_results_oracle.tex <==
\begin{table}[t!]
\centering
\footnotesize
\begin{tabular}{lcc}
\toprule
\textbf{Dataset} & \textbf{GeNER} & \textbf{HighGEN} \\
\midrule
CoNLL-2003 & 71.0 (73.1/69.0) & \textbf{72.1} (74.5/69.8) \\
Wikigold & 72.5 (65.8/79.9) & \textbf{73.4}
 (72.3/74.5) \\
WNUT-16 & \textbf{48.5} (44.8/54.0) & 46.7 (40.9/54.6) \\
NCBI-disease & 67.9 (75.0/62.1) & \textbf{72.5} (77.6/68.0) \\
BC5CDR & 74.3 (71.9/76.8) & \textbf{76.5} (79.1/74.2) \\
CHEMDNER & 62.3 (60.3/64.4) & \textbf{64.3} (57.4/73.2) \\
\midrule
Average & 66.1 (65.2/67.7) & \textbf{67.6} (67.0/69.1) \\
\bottomrule
\end{tabular}
\caption{asdf}
\label{table:bond_results_oracle}
\end{table}

==> tables/motivating_example.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{adjustbox}{max width = 0.99\columnwidth}
\begin{tabular}{c|cc}
\toprule
 & \multicolumn{2}{c}{Which \typetoken?} \\
Rank & disease & sports player \\
\midrule
1 & syphilis (88) & cristiano ronaldo (246) \\
2 & leprosy (87) & lionel messi (128)  \\
3 & typhus (82) & ronaldo (58) \\
4 & smallpox (79) & pelé (57)  \\
5 & tuberculosis (78) & roger federer (52) \\
6 & polio (65) & david beckham (49) \\
7 & cholera (57) & ronaldinho (32) \\
8 & aids (44) & zinedine zidane (17) \\
9 & measles (28) & franz beckenbauer (17) \\
10 & parkinson's disease (25) & thierry henry (13) \\
\midrule
Sum & 633 & 669 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{
top 1,000 phrases from 2018-12-20 Wikipedia for the questions ``Which disease?'' and ``Which sports player?.''
Generated dictionaries contain many of the same entities.
}
\label{tab:motivating_example}
\end{table}

==> tables/search_dict_size.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{ll}
\toprule
\textbf{Dataset} & \boldsymbol{$k^{\prime}_l$} \textbf{(\# of Retrieved Phrases)} \\
\midrule
\multicolumn{2}{l}{\textit{Self-training}} \\
\midrule
CoNLL-2003 & $\{$5k, 10k, $\dots$, \textbf{30k}, 35k$\}$  \\
Wikigold & $\{$1.5k, 3k, \textbf{4.5k}, $\dots$, 7.5k$\}$ \\
WNUT-16 & $\{$1k, 2k, \textbf{3k}, $\dots$, 6k$\}$ \\
NCBI-disease & $\{$10k, 20k, $\dots$, \textbf{50k}, $\dots$, 90k$\}$   \\
BC5CDR & $\{$10k, 20k, \textbf{30k}, $\dots$, 90k$\}$ \\
CHEMDNER & $\{$10k, \textbf{20k}, 30k, 40k$\}$  \\
\midrule
\multicolumn{2}{l}{\textit{Standard}} \\
\midrule
CoNLL-2003 & $\{$5k, 10k, $\dots$, \textbf{25k}, 30k, 35k$\}$  \\
Wikigold & $\{$1.5k, 3k, \textbf{4.5k}, $\dots$, 7.5k$\}$ \\
WNUT-16 & $\{$1k, 2k, $\dots$, \textbf{5k}, 6k$\}$ \\
NCBI-disease & $\{$10k, 20k, $\dots$, \textbf{80k}, 90k$\}$   \\
BC5CDR & $\{$10k, 20k, $\dots$, \textbf{50k}, $\dots$, 90k$\}$ \\
CHEMDNER & $\{$\textbf{10k}, 20k, 30k, 40k$\}$  \\
\bottomrule
\end{tabular}
\caption{
Hyperparameter bounds for obtaining obtimal dictionary sizes ($k^{\prime}_l$).
Best dictionary sizes are represented in bold.
}
\label{tab:search_dict_size}
\end{table}

==> tables/self_training_hyperparams.tex <==
\begin{table}[t!]
\centering
\footnotesize
\begin{tabular}{lcc}
\toprule
\textbf{Dataset} & \boldsymbol{$T_\text{begin}$} & \boldsymbol{$T_\text{update}$}  \\
\midrule
CoNLL-2003 & 900 & 300  \\
Wikigold & 500 & 200  \\
WNUT-16 & 900 & 450  \\
NCBI-disease & 900 & 300  \\
BC5CDR & 500 & 200  \\
CHEMDNER & 900 & 300  \\
\bottomrule
\end{tabular}
\caption{
Hyperparameter configuration of our self-training models.
}
\label{tab:self_training_config}
\end{table}
